On the Stochastic Analysis of a Quantum Entanglement Switch

We study a quantum entanglement switch that serves $k$ users in a star topology. We model variants of the system using Markov chains and standard queueing theory and obtain expressions for switch capacity and the expected number of qubits stored in memory at the switch. While it is more accurate to use a discrete-time Markov chain (DTMC) to model such systems, we quickly encounter practical constraints of using this technique and switch to using continuous-time Markov chains (CTMCs). Using CTMCs allows us to obtain a number of analytic results for systems in which the links are homogeneous or heterogeneous and for switches that have infinite or finite buffer sizes. In addition, we can model the effects of decoherence of quantum states fairly easily using CTMCs. We also compare the results we obtain from the DTMC against the CTMC in the case of homogeneous links and infinite buffer, and learn that the CTMC is a reasonable approximation of the DTMC. From numerical observations, we discover that decoherence has little effect on capacity and expected number of stored qubits for homogeneous systems. For heterogeneous systems, especially those operating close to stability constraints, buffer size and decoherence can have significant effects on performance metrics. We also learn that in general, increasing the buffer size from one to two qubits per link is advantageous to most systems, while increasing the buffer size further yields diminishing returns.

==> CTMCBipartiteApp.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = quantum-sigconf.tex
\subsection{Homogeneous Links}
\label{app:homogInfBufCTMC}
These derivations are for Section \ref{sec:analysisHomogCTMC}.
\subsubsection{Infinite Buffer}
From (\ref{eq:ctmc1}) and (\ref{eq:ctmc2}), we obtain
\begin{align*}
\pi_1 &= \frac{k}{k-1}\pi_0,\\
\pi_i &= \frac{1}{k-1}\pi_{i-1}=\left(\frac{1}{k-1}\right)^{i-1}\pi_1=k\left(\frac{1}{k-1}\right)^{i}\pi_0,~i=2,3,\dots
\end{align*}
We can solve for $\pi_0$ using the normalizing constraint (\ref{eq:ctmc3}):
\begin{align*}
\pi_0+\sum\limits_{i=1}^{\infty}k\left(\frac{1}{k-1}\right)^{i}\pi_0 &=1,\\
\pi_0+k\pi_0\sum\limits_{i=1}^{\infty}\left(\frac{1}{k-1}\right)^{i} &=1,\\
\pi_0+k\pi_0\left(\sum\limits_{i=0}^{\infty}\left(\frac{1}{k-1}\right)^{i}-1\right) &=1.
\end{align*}
For $k\geq 3$ (which is the stability condition for this CTMC), we can write
\begin{align*}
\pi_0+k\pi_0\left(\frac{1}{1-\frac{1}{k-1}}-1\right) &=1,\\
%\pi_0+k\pi_0\left(\frac{k-1}{k-2}-1\right) &=1,\\
\pi_0+\pi_0\left(\frac{k}{k-2}\right) &=1,\text{~and therefore,}\\
%\end{align*}
%\begin{flalign*}
\pi_0 &= %\frac{1}{1+\frac{k}{k-2}}=\frac{k-2}{2k-2}=
\frac{k-2}{2(k-1)}.
\end{align*}
\subsubsection{Finite Buffer}
From the balance equations, we have
\begin{align*}
\pi_1 &= \frac{k}{k-1}\pi_0,~ \pi_i = k\left(\frac{1}{k-1}\right)^i\pi_0,~i=2,\dots,B.
\end{align*}
To solve for $\pi_0$, we use the normalizing constraint. Let $\rho\coloneqq 1/(k-1)$. Then
\begin{align*}
\pi_0+k\pi_0\sum\limits_{i=1}^B \rho^i &=1,\\
\pi_0\left(1+k\left(\sum\limits_{i=0}^B \rho^i-1\right)\right) &=1,\\
\pi_0\left(1+k\left(\frac{1-\rho^{B+1}}{1-\rho}-1\right)\right) &=1,
\end{align*}
and
\begin{align*}
\pi_0 &= \left(1+k\left(\frac{1-\rho^{B+1}}{1-\rho}-1\right)\right)^{-1}\\
  &= \left(1+k\left(\frac{\rho-\rho^{B+1}}{1-\rho}\right)\right)^{-1}\\
    &= \left(1+k\left(\frac{\rho(1-\rho^{B})}{1-\rho}\right)\right)^{-1}
    = \left(1+k\left(\frac{1-\rho^{B}}{(k-1)\left(1-\frac{1}{k-1}\right)}\right)\right)^{-1}\\
    &= \left(1+\frac{k-k\rho^{B}}{k-2}\right)^{-1}
    =\left(\frac{2(k-1)-k\rho^{B}}{k-2}\right)^{-1}\\
    &=\frac{k-2}{2(k-1)-k\left(\frac{1}{k-1}\right)^B}\\
    &=\frac{(k-2)(k-1)^B}{2(k-1)^{B+1}-k}.
\end{align*}

==> CTMCTripartite.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = quantum-sigconf.tex
\label{sec:CTMCTripartite}
Consider a switch that exclusively serves tripartite entanglements to its users, \emph{i.e.}, whenever there are enough available link entanglements, the switch performs 3-way GHZ measurements according to the OLEF policy. We assume that at any time, any triplet of users wishes to ``communicate'', or share an entangled state. In this work, we consider the simplest variant of this system, in which all links are homogeneous and the switch has infinite buffer. Note that in such a system, at most two links can have stored entanglements at any given time; therefore, the state space of the CTMC is given by $(N_1,N_2)\in\{0,1,2,\dots\}^2$, where $N_i$, $i=1,2$, is the number of entanglements stored for the two links. State $(0,0)$ corresponds to the case where no links have entanglements, and any state $(j,0)$ or $(0,j)$, $j\geq1$, corresponds to cases where only one link has stored entanglements.
\begin{figure}[h]
\centering
\includegraphics[width=0.35\textwidth,trim={1.8cm 0.7cm 0.6cm 0},clip]{tripartCTMC.pdf}
\caption{CTMC for a system with $k$ homogeneous links and a switch that has infinite buffer and serves only tripartite entanglements. $\mu$ is the entanglement generation rate.}
\label{fig:ctmcTripart}
\end{figure}

Figure \ref{fig:ctmcTripart} presents one possible construction of a CTMC for this system. Note that in theory, states $(i,j)$ and $(j,i)$, for $i,j\in\{0,1,2,\dots\}$ are equivalent. We choose to differentiate between them because it simplifies the analysis of the model, despite increasing the number of total states in the CTMC. Consider state $(0,0)$. From there, an entanglement is generated with rate $k\mu$; hence, we split this rate in half among the states $(0,1)$ and $(1,0)$. The remaining transitions in this CTMC are analogous to those of a model of a switch serving bipartite entanglements to homogeneous links. Note that whenever two distinct links have at least one entanglement stored each, a GHZ measurement is performed with rate $(k-2)\mu$, which is the rate at which one of the other $k-2$ links generates an entanglement.

The analysis of this system is challenging in that we cannot directly obtain its stationary distribution. However, we can still obtain  system capacity by taking advantage of the chain's structure and homogeneity of the links. To simplify the analysis, let $\lambda= \mu$ and $\nu=(k-2)\mu$. We assume that $k\geq 3$ (we will show later on that the Markov chain is not positive recurrent if $k=3$). In this notation, note that $\frac{k}{2}\mu=\frac{2\lambda+\nu}{2}$ and $(k-1)\mu=\lambda+\nu$.

The non-zero transition rates are
\begin{eqnarray*}
&& (0,0) \to (1,0) \quad \hbox{ with rate } \frac{2\lambda+\nu}{2}, \\
&& (0,0) \to (0,1) \quad \hbox{ with rate } \frac{2\lambda+\nu}{2}, \\
&\hbox{For } i\geq 1: & (i,0)\to (i,1) \quad \hbox{ with rate } \lambda+\nu,\\
&\hbox{For } j\geq 1: & (0,j)\to (1,j) \quad \hbox{ with rate  }\lambda+\nu,\\
&\hbox{For } i\geq 1:& (i,0)\to (i+1,0) \quad \hbox{ with rate } \lambda,\\
&\hbox{For }j\geq 1 :& (0,j)\to (0,j+1) \quad \hbox{ with rate } \lambda,\\
%&\hbox{For } i\geq 1, j\geq 0:& (i,j)\to (i,j+1) \quad \hbox{ with rate } \lambda\\
&\hbox{For } i\geq 1, j\geq 1:& (i,j)\to (i,j+1) \quad \hbox{ with rate } \lambda,\\
%&\hbox{For } i\geq 0,  j\geq 1: & (i,j)\to (i+1,j) \quad \hbox{ with rate } \lambda\\
&\hbox{For } i\geq 1,  j\geq 1: & (i,j)\to (i+1,j) \quad \hbox{ with rate } \lambda,\\
&\hbox{For } i\geq 1, j\geq 1:&(i,j)\to (i-1,j-1)\quad \hbox{ with rate } \nu.
\end{eqnarray*}
Let $\pi(i,j)$ be the steady-state probability that the chain is in state $(i,j)$.  The balance equations are 
\begin{align}
(2\lambda+\nu)\pi(0,0)&= \nu \pi(1,1),\label{baleq-1}\\
(2\lambda+\nu)\pi(1,0)&=   \frac{(2\lambda+\nu)}{2} \pi(0,0)+\nu\pi(2,1),  \label{baleq-2}\\
(2\lambda+\nu)\pi(0,1)&=   \frac{(2\lambda+\nu)}{2} \pi(0,0)+\nu\pi(1,2), \label{baleq-3}\\
(2\lambda+\nu)\pi(1,1)&= \nu \pi(2,2) + (\lambda + \nu) \pi(1,0) + (\lambda +\nu) \pi(0,1), \label{baleq-4}\\ 
(2\lambda+\nu)\pi(i,0)&= \nu \pi(i+1,1)+\lambda \pi(i-1,0),\quad i\geq 2,\label{baleq-5}\\
(2\lambda+\nu)\pi(0,j)&= \nu \pi(1,j+1)+\lambda \pi(0,j-1),\quad j\geq 2,\label{baleq-6}\\
(2\lambda+\nu)\pi(i,1)&=\nu \pi(i+1,2)+\lambda\pi(i-1,1)+(\lambda+\nu)\pi(i,0),\nonumber\\ 
&\hskip0.28\textwidth i\geq 2,\label{baleq-7}\\
(2\lambda+\nu)\pi(1,j)&=\nu \pi(2,j+1)+(\lambda+\nu)\pi(0,j)+\lambda\pi(1,j-1),\nonumber\\
&\hskip0.28\textwidth j\geq 2,\label{baleq-8}\\
(2\lambda+\nu)\pi(i,j)&=\nu \pi(i+1,j+1)+\lambda\pi(i-1,j)+\lambda\pi(i,j-1),\nonumber\\
&\hskip0.24\textwidth i\geq 2, j\geq 2.\label{baleq-9}
\end{align}
In the following discussion, we use the definition $0^0\coloneqq1$.
%\begin{align*}
%0^0 \coloneqq \lim_{\substack{x\to0,\\ x>0}} x^x = \lim_{\substack{x\to 0,\\ x>0}}e^{x\log(x)}=1.
%\end{align*}
Define the generating function
\[
%F(x,y)\coloneqq \sum_{i\geq 0\atop j\geq 0} \pi(i,j) x^i y^j,\quad |x|\leq 1,\, |y|\leq  1.
F(x,y)\coloneqq \sum_{i,j\geq 0} \pi(i,j) x^i y^j,\quad |x|\leq 1,\, |y|\leq  1.
\]
It is shown in Lemma \ref{lem:appA} in Appendix \ref{app:ctmcTripartite} that for $|x|\leq 1,|y|\leq 1,$
%\footnote{As a sanity check, note that both sides of this equation vanish when $(x,y)=(1,1)$. Also, notice that when we multiply both sides of this equation by $xy$ and let $(x,y)=(0,0)$ then both sides of the resulting equation are equal (they are equal to $-\nu F(0,0)$).}
\begin{align}
\hspace{-2em}K(x,y)F(x,y)=a(x,y)F(x,0)+b(x,y)F(0,y)+c(x,y)F(0,0),\hspace{-1.5em}\label{eq:F}
\end{align}
\vspace{-1.4em}
\begin{align*}
\text{where}\quad
K(x,y)&\coloneqq\lambda(1-x)+\lambda(1-y)+\nu\left(1-\frac{1}{xy}\right),\\%\label{def:T}\\
a(x,y)&\coloneqq\nu\left(y-\frac{1}{xy}\right),\\%   \label{def:a} \\
b(x,y)&\coloneqq\nu\left(x-\frac{1}{xy}\right), \quad\text{and}\\%   \label{def:b}\\ 
c(x,y)&\coloneqq-\nu\left(\frac{x+y}{2}-\frac{1}{xy}\right).% \label{def:c}
\end{align*}
Now, note that a GHZ measurement can be generated from any state $(i,j)$ for $i,j\geq 1$: this occurs with rate $\nu=(k-2)\mu$, whenever a third link (not one of the two links that has a stored entanglement) generates an entanglement. Hence, the system capacity $C$ is 
\begin{align}
C&=q\nu \sum_{i\geq 1\atop j\geq 1}\pi(i,j)\nonumber \\
&= q\nu (1-F(1,0)-F(0,1)+F(0,0))\nonumber\\
& = q\mu (k-2) (1-2F(1,0)+F(0,0)),
\label{capacity}
\end{align}
since (see Eq. (\ref{eq:F})) $F(x,y)=F(y,x)$  for all $|x|\leq 1$, $|y|\leq 1$.

Assume for now that $k\geq 4$ so that $\lambda\not=\nu$.
When $K(x,x)\not=0$, Eq. (\ref{eq:F}) can be rewritten as
\begin{equation}
\label{Fxx}
F(x,x) =\frac{a(x,x)+b(x,x)}{K(x,x)} F(x,0)+ \frac{c(x,x)}{K(x,x)}F(0,0),
\end{equation}
where we have used the identity $F(x,0)=F(0,x)$. Letting $x\to 1$ in (\ref{Fxx}), we get by L'H\^opital's rule 
\[
1=\frac{3\nu}{\nu-\lambda} F(1,0)-\frac{3\nu}{2(\nu-\lambda)}F(0,0), \quad\text{yielding}
\]
\begin{equation}
\label{eq:F00-1}
F(0,0)-2F(1,0)= -\frac{2(k-3)}{3(k-2)},
\end{equation}
when $k\geq 4$.
By introducing Eq. (\ref{eq:F00-1}) into Eq. (\ref{capacity}) we get
\begin{equation}
\label{value-C}
C=\frac{ qk\mu }{3}.
\end{equation}

Assume now that $k=3$, namely, $\lambda=\nu$. In this case, $K(x,x)$ has a zero of order two at $x=1$. More precisely, $K(x,x)=-3\nu (x-1)^2 +o((x-1)^2)$.
Since $F(1,1)=1$, this necessarily implies that the derivative of $(a(x,x)+b(x,x))F(x,0)+c(x,x)F(0,0)$ vanishes when $x=1$. This derivative equals $\nu(2F(1,0)-F(0,0))$. Hence,
$F(0,0)=2F(1,0)$. 
%Notice that the pair $(F(1,0),F(0,0))=(0,0)$ is a solution of (\ref{eq:F00-2}). 
Assume that the latter identity holds,  and let us calculate
\begin{align}
\lim_{x\to 1}G(x) \coloneqq
\lim_{x\to 1}\frac{(a(x,x)+b(x,x))F(x,0)+ c(x,x)F(0,0)}{K(x,x)}. 
\label{eq:limTri}
\end{align}
By performing a second-order Taylor series expansion of the numerator of (\ref{eq:limTri}) at $x=1$, we obtain
\begin{align*}
%&\lim_{x\to 1}\frac{(a(x,x)+b(x,x))F(x,0)+ c(x,x)F(0,0)}{K(x,x)}=\\
\lim_{x\to 1}G(x)=
\lim_{x\to 1}\frac{6\nu F'(1,0)(x-1)^2 +o((x-1)^2)}{-3\nu (x-1)^2 +o((x-1)^2)}=-2 F'(1,0),
\end{align*}
%we obtain that $\lim_{x\to 1}\frac{(a(x,x)+b(x,x))F(x,0)+ c(x,x)F(0,0)}{K(x,x)}=-2 F'(1,0)$, 
with $F'(1,0)\coloneqq\frac{dF(x,0)}{dx}\Big|_{x=1}$. Hence, $F(1,1)=1= -2 F'(1,0)$ which is not possible as
$F'(1,0)\geq 0$.  We conclude
that $F(x,y)$ cannot satisfy Eq. (\ref{eq:F}), which implies that the (irreducible) Markov chain is not positive recurrent when $k=3$. Therefore, $F(0,0)=F(1,0)=0$ and 
\begin{equation}
\label{valueC-k=3}
C=q\mu.
\end{equation}
From Eqs. (\ref{value-C}) and (\ref{valueC-k=3}), we conclude that for $k\geq 3$, the capacity of a homogeneous system with infinite buffer and tripartite entanglement switching is $qk\mu/3$.

In principle Eq. (\ref{eq:F}) can be solved by using the theory developed in \cite{FI-79, CB-83}), which consists of reducing it to
the solution of a Riemann-Hilbert boundary problem on a closed curve. Solving (\ref{eq:F}) was not required here as the capacity
could be obtained by letting $(x,x)=(x,y)$ in (\ref{eq:F}) and then $x\to 1$.

==> CTMCTripartiteCapApp.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = quantum-sigconf.tex
\label{app:ctmcTripartite}
Following are derivations for the capacity of a switch that serves only tripartite entanglements in a system with homogeneous links.
\begin{lem}
\label{lem:appA}
For all $|x|\leq 1$, $|y|\leq 1$, the generating function $F(x,y)$ satisfies the functional equation
\[
K(x,y)F(x,y)=a(x,y)F(x,0)+b(x,y)F(0,y)+c(x,y)F(0,0),
\]
where 
\begin{align*}
K(x,y)&\coloneqq \lambda(1-x)+\lambda(1-y)+\nu\left(1-\frac{1}{xy}\right),\\
a(x,y)&\coloneqq\nu\left(y-\frac{1}{xy}\right), \\  
b(x,y)&\coloneqq \nu\left(x-\frac{1}{xy}\right),\quad\text{and} \\ 
c(x,y)&\coloneqq  -\nu\left(\frac{x+y}{2}-\frac{1}{xy}\right).
\end{align*}
\end{lem}
%
\begin{proof} Note that $\pi(0,0)=F(0,0)$.
We will need the following identities:
\begin{align}
&\sum_{i\geq 1\atop j\geq 1}\pi(i,j)x^iy^j = F(x,y)-F(x,0)-F(0,y)+ F(0,0),\label{id-1}\\
&\sum_{i\geq 0\atop j\geq 1}\pi(i,j)x^iy^j = F(x,y)-F(x,0),\label{id-2}\\
&\sum_{i\geq 1\atop j\geq 0}\pi(i,j)x^iy^j = F(x,y)-F(0,y),\label{id-3}\\
&\sum_{i\geq 2\atop j\geq 2} \pi(i,j)x^i y^j= F(x,y)-F(x,0)-F(0,y)+F(0,0)\nonumber\\
& -y\sum_{i\geq 1}\pi(i,1)x^i - x\sum_{j\geq 1}\pi(1,j)y^j +\pi(1,1)xy, \label{id-4}\\
&\sum_{i\geq 3\atop j\geq 3} \pi(i,j)x^i y^j=\sum_{i\geq 2\atop j\geq 2} \pi(i,j)x^i y^j -x^2\sum_{j\geq 2} \pi(2,j)y^j\nonumber\\
& -y^2\sum_{i\geq 2} \pi(i,2)x^i+x^2y^2\pi(2,2)\nonumber\\
&=F(x,y)-F(x,0)-F(0,y)+F(0,0) -y\sum_{i\geq 1}\pi(i,1)x^i\nonumber\\
&- x\sum_{j\geq 1}\pi(1,j)y^j
-x^2\sum_{j\geq 2} \pi(2,j)y^j -y^2\sum_{i\geq 2} \pi(i,2)x^i\nonumber\\
&+xy\pi(1,1) +x^2y^2\pi(2,2),\label{id-5}
\end{align}
where the latter equality comes from  (\ref{id-4}).
Multiplying both sides of Eq. (\ref{baleq-5}) by $x^i$ and then summing over all $i\geq 2$ yields
\begin{align}
(2\lambda+\nu)\sum_{i\geq 2}\pi(i,0)x^i&= \frac{\nu}{x}\sum_{i\geq 2} \pi(i+1,1) x^{i+1} +\lambda x\sum_{i\geq 2} \pi(i-1,0)x^{i-1}\nonumber\\
&=\frac{\nu}{x}\sum_{i\geq 3} \pi(i,1) x^{i} +\lambda x\sum_{i\geq 1} \pi(i,0)x^{i}\nonumber\\
&=\frac{\nu}{x}\left(\sum_{i\geq 1} \pi(i,1) x^{i}- \pi(2,1) x^2 - \pi(1,1)x\right)\nonumber\\
&+\lambda x (F(x,0)-\pi(0,0))    .\label{eq1}
\end{align}
Since $\sum_{i\geq 2}\pi(i,0)x^i=F(x,0)- \pi(1,0)x - \pi(0,0)$, we obtain the following from Eq. (\ref{eq1}) by using (\ref{baleq-1}) and (\ref{baleq-2}):
%\begin{framed}
\begin{equation}
\label{eq2}
\frac{\nu}{x}\sum_{i\geq 1} \pi(i,1) x^{i}  = (\lambda+\lambda(1-x)+\nu)F(x,0) - \frac{\nu x}{2} \pi(0,0),\quad |x|\leq 1,
\end{equation}
%\end{framed}
Similarly, from Eq. (\ref{baleq-6}) we obtain by using  (\ref{baleq-1}) and (\ref{baleq-3})
%\begin{framed}
\begin{equation}
\frac{\nu}{y}\sum_{j\geq 1} \pi(1,j) y^{j} = (\lambda+\lambda(1-y)+\nu)F(0,y)-\frac{\nu y}{2}\pi(0,0),\quad |y|\leq 1.
\label{eq3}
\end{equation}
%\end{framed}
Multiplying now both sides of Eq. (\ref{baleq-7}) by $x^i$ and then summing over all $i\geq 2$, gives
\begin{align*}
&(2\lambda+\nu)\sum_{i\geq 2}\pi(i,1)x^i=\frac{\nu}{x}\sum_{i\geq 2}\pi(i+1,2)x^{i+1}\\
&+\lambda x\sum_{i\geq 2}\pi(i-1,1)x^{i-1}+(\lambda+\nu)\sum_{i\geq 2}\pi(i,0)x^i\nonumber\\
&= \frac{\nu}{x}\sum_{i\geq 3}\pi(i,2)x^{i}+\lambda x\sum_{i\geq 1}\pi(i,1)x^{i}+(\lambda+\nu)\sum_{i\geq 2}\pi(i,0)x^i\nonumber\\
&=  \frac{\nu}{x}\left(  \sum_{i\geq 1}\pi(i,2)x^{i} -\pi(2,2)x^2- \pi(1,2)x\right)+\lambda x\sum_{i\geq 1}\pi(i,1)x^{i}\nonumber\\
&+(\lambda+\nu)\left(\sum_{i\geq 0}\pi(i,0)x^i-\pi(1,0)x - \pi(0,0)\right).
\end{align*}
With $\sum_{i\geq 2}\pi(i,1)x^i=\sum_{i\geq 1}\pi(i,1)x^i- \pi(1,1)x$, we find
\begin{align*}
&(\lambda+\lambda(1-x)+\nu)\sum_{i\geq 1}\pi(i,1)x^i =\frac{\nu}{x}\sum_{i\geq 1}\pi(i,2)x^{i}\\
& -\nu x\pi(2,2)-\nu\pi(1,2)
 +(\lambda+\nu)F(x,0)-(\lambda+\nu)x\pi(1,0)\\
&-(\lambda+\nu)\pi(0,0)+ (2\lambda +\nu)x\pi(1,1)
\end{align*}
or
%\begin{framed}
\begin{align}
\frac{\nu}{x}\sum_{i\geq 1}\pi(i,2)x^{i}&= (\lambda+\lambda(1-x)+\nu)\sum_{i\geq 1}\pi(i,1)x^i +\nu x\pi(2,2)\\
&+\nu\pi(1,2)
 -(\lambda+\nu)F(x,0)+(\lambda+\nu)x\pi(1,0)\nonumber\\
&+(\lambda+\nu)\pi(0,0)- (2\lambda +\nu)x\pi(1,1),\quad |x|\leq 1.
\label{eq4}
\end{align}
%\end{framed}
Similarly,
%\begin{framed}
\begin{align}
\frac{\nu}{y}\sum_{j\geq 1}\pi(2,j)y^{j}&= (\lambda+\lambda(1-y)+\nu)\sum_{j\geq 1}\pi(1,j)y^j +\nu y\pi(2,2)\\
&+\nu\pi(2,1) -(\lambda+\nu)F(0,y)+(\lambda+\nu)y\pi(0,1)\nonumber\\
&+(\lambda+\nu)\pi(0,0)- (2\lambda +\nu)y\pi(1,1),\quad |y|\leq 1.
\label{eq5}
\end{align}
%\end{framed}
Multiplying now both sides of Eq. (\ref{baleq-9}) by $x^i y^j$ and then summing over all $i\geq 2$, $j\geq 2$, yields
\begin{align}
&(2\lambda+\nu)\sum_{i\geq 2\atop j\geq 2}\pi(i,j)x^i y^j = \frac{\nu}{xy}\sum_{i\geq 2\atop j\geq 2}\pi(i+1,j+1)x^{i+1} y^{j+1}\nonumber\\
&+\lambda x \sum_{i\geq 2\atop j\geq 2} \pi(i-1,j)x^{i-1}y^j +\lambda y \sum_{i\geq 2\atop j\geq 2} \pi(i,j-1)x^i y^{j-1} \nonumber\\
&=  \frac{\nu}{xy}\sum_{i\geq 3\atop j\geq 3}\pi(i,j)x^{i} y^{j}+\lambda x \sum_{i\geq 1\atop j\geq 2} \pi(i,j)x^i y^j +\lambda y \sum_{i\geq 2\atop j\geq 1} \pi(i,j)x^i y^j.
\label{eq6}
\end{align}
By using identities (\ref{id-1})-(\ref{id-5}), Eq. (\ref{eq6}) rewrites
\begin{align}
&(2\lambda+\nu)\left[F(x,y)-F(x,0)-F(0,y)+F(0,0)-y\sum_{i\geq 1}\pi(i,1)x^i \right.\nonumber\\
&-\left. x\sum_{j\geq 1}\pi(1,j)y^j +\pi(1,1)xy\right]\nonumber\\
&=\left(\lambda(x+y)+\frac{\nu}{xy}\right)\left[F(x,y)-F(x,0)-F(0,y)+F(0,0)\right ]\nonumber\\
&-\left(\lambda xy+\frac{\nu}{x} \right)\sum_{i\geq 1}\pi(i,1)x^i -\left(\lambda xy+\frac{\nu}{y}\right)\sum_{j\geq 1}\pi(1,j)y^j\nonumber\\ 
&-\frac{\nu y}{x} \sum_{i\geq 2} \pi(i,2)x^i -\frac{\nu x}{y} \sum_{j\geq 2} \pi(2,j)y^j%  \nonumber\\
+\nu \pi(1,1)+\nu xy \pi(2,2). \label{eq7}
\end{align}
Simple algebra in (\ref{eq7}) gives
\begin{align*}
&\left(\lambda(1-x)+\lambda(1-y)+\nu \left(1-\frac{1}{xy}\right)\right)\left[F(x,y)-F(x,0)\right.\\
&\hskip0.25\textwidth\left.-F(0,y)+F(0,0)\right]\\
&= \left((2\lambda+\nu)y-\lambda x y -\frac{\nu}{x}\right) \sum_{i\geq 1} \pi(i,1)x^i\\
&+ \left((2\lambda+\nu)x-\lambda x y-\frac{\nu}{y}\right) \sum_{j\geq 1} \pi(1,j)y^j\\
&-\frac{\nu y}{x} \sum_{i\geq 1} \pi(i,2)x^i - \frac{\nu x }{y} \sum_{j\geq 1} \pi(2,j)y^j\\
&-((2\lambda+\nu)xy-\nu)\pi(1,1)+\nu y\pi(1,2)+\nu x\pi(2,1)+\nu xy \pi(2,2)\\
&= -\frac{\nu}{x} \sum_{i\geq 1}\pi(i,1)x^i -\frac{\nu}{y}\sum_{j\geq 1}\pi(1,j)y^j\\
&+(\lambda+\nu)y F(x,0)+(\lambda+\nu)x F(0,y)\\
&-\nu xy \pi(2,2) +((2\lambda+\nu)xy +\nu)\pi(1,1)\\
&-(\lambda+\nu)xy (\pi(1,0)+\pi(0,1)) - (\lambda+\nu)(x+y)\pi(0,0),
\end{align*}
where we have used (\ref{eq4}) and (\ref{eq5}) to derive the last equality. Using (\ref{eq2}) and (\ref{eq3}), we now obtain
\begin{align}
&\left(\lambda(1-x)+\lambda(1-y)+\nu \left(1-\frac{1}{xy}\right)\right)\left[F(x,y)-F(x,0)\right.\nonumber\\
&\hskip0.25\textwidth\left.-F(0,y)+F(0,0)\right]\nonumber\\
&=-\left(\lambda(1-x)+(\lambda+\nu)(1-y)\right)F(x,0)\nonumber\\
&-\left(\lambda(1-y)+(\lambda+\nu)(1-x)\right)F(0,y)\nonumber\\
& -\left(\frac{2\lambda+\nu}{2}\right) (x+y) \pi(0,0) +d(x,y),\label{eq10}
\end{align}
with
\begin{align}
d(x,y)&\coloneqq \nu \pi(1,1)+xy\left(-\nu \pi(2,2)+(2\lambda+\nu)\pi(1,1)\right.\nonumber\\
&\hskip0.12\textwidth\left.-(\lambda+\nu)\pi(1,0) -(\lambda+\nu)\pi(0,1)\right).\label{def:d}
\end{align}
From (\ref{baleq-4}), we see that the second term in the right-hand side of (\ref{def:d}) is equal to zero, so that
\begin{equation}
d(x,y)=\nu\pi(1,1)= (2\lambda+\nu)\pi(0,0)
\label{eq11}
\end{equation}
where the second equality comes from (\ref{baleq-1}). Collecting terms having $F(x,0)$, $F(0,y)$, and $F(0,0)$ as factors in (\ref{eq10}) and using (\ref{eq11}) finally yields
\begin{align*}
&\left(\lambda(1-x)+\lambda(1-y)+\nu \left(1-\frac{1}{xy}\right)\right)F(x,y)=\\
&\nu\left(y-\frac{1}{xy}\right)F(x,0)+\nu\left(x-\frac{1}{xy}\right)F(0,y) -\nu\left(\frac{x+y}{2}-\frac{1}{xy}\right)F(0,0),
\end{align*}
which concludes the proof.
\end{proof}

==> Conjecture.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = quantum-sigconf.tex
\label{sec:conj}
In Section \ref{sec:ctmcInfBufHomog}, we showed that the capacity of an infinite buffer switch system with homogeneous  links serving bipartite entanglements is $qk\mu/2$. In Section \ref{sec:CTMCTripartite}, we showed that a similar switch serving tripartite entanglements has capacity $qk\mu/3$, under the assumption that measurement success probabilities are the same. For the former system, the state space consisted of one variable: a single link that is associated with stored (or unused) entanglements. For the latter system, one must keep track of at least two such links. Similarly, to model a system in which the switch serves $n$-partite entanglements to users, one would have to keep track of a vector of dimension $n-1$. As $n$ increases, it becomes increasingly more challenging to model and analyze an $n$-partite entanglement switching system, even in the simplest case of homogeneous links and infinite buffer. Indeed, even in the case of $n=3$, we did not pursue the difficult task of obtaining the stationary distribution for the system and instead derived the capacity directly.

While deriving an expression for capacity can be involved, the results we obtained for $n=2$ and $n=3$ are simple and intuitive: in the numerator, we have $k\mu$, which is the aggregate successful entanglement generation rate of all $k$ links. Each measurement consumes $n$ of these entanglements; hence, we divide $k\mu$ by $n$, for $n=2,3$, and since measurements succeed with probability $q$, multiply by $q$. For $n=2$, we also have the discrete analogue: the expected number of successful entanglements after one time step is $kp$, so the capacity is $qkp/2$ (proven in Section \ref{sec:dtmcAnalysis}). One may then ask the following: ``What is the maximum capacity of a homogeneous system with an infinite-buffer switch serving $n$-partite entanglements, for $n\geq 2$?'' Using the same reasoning as for $n=2$ and $3$, we conjecture that the capacity is $qk\mu/n$ for all $n\geq 2$. Note that capacity, by its definition, is an expected value: it is the sum of $n$-partite measurement generation rates, each weighted by the steady-state probability of the state from which the measurement is generated. Hence, it would not make sense for capacity to exceed $qk\mu/n$. Because of this, we further conjecture that for the system described here, OLEF is optimal in that it maximizes capacity.
